Few-Shot Semantic Segmentation Augmented with Image-Level Weak Annotations

Despite the great progress made by deep neural networks in the semantic segmentation task, traditional neural-networkbased methods typically suffer from a shortage of large amounts of pixel-level annotations. Recent progress in fewshot semantic segmentation tackles the issue by only a few pixel-level annotated examples. However, these few-shot approaches cannot easily be applied to multi-way or weak annotation settings. In this paper, we advance the few-shot segmentation paradigm towards a scenario where image-level annotations are available to help the training process of a few pixel-level annotations. Our key idea is to learn a better prototype representation of the class by fusing the knowledge from the image-level labeled data. Specifically, we propose a new framework, called PAIA, to learn the class prototype representation in a metric space by integrating image-level annotations. Furthermore, by considering the uncertainty of pseudo-masks, a distilled soft masked average pooling strategy is designed to handle distractions in image-level annotations. Extensive empirical results on two datasets show superior performance of PAIA.

==> Related.tex <==
\section{Related Work}\label{section:related_work}

\subsection{Weakly- and Semi-supervised Segmentation}
In light of the expensive cost of annotated pixel-level labels, the segmentation task has recently received increasing interest in the semi-and weakly-supervised training schemes. Weakly-supervised methods aim to use weak labels like image-level class labels~\cite{papandreou2015weakly,hong2016learning} and bounding boxes~\cite{dai2015boxsup,khoreva2017simple} to train the segmentation model, achieving the similar performance as supervised models.
And the general idea of existing works on the semi-supervised segmentation task can be largely grouped into two types: one is to employ a GAN-based method that generates additional images for training~\cite{souly2017semi,hung2018adversarial,sankaranarayanan2018learning,xue2018segan}, the other is to generate pseudo-labels for the image-level labeled data which can be used to train the model as full supervision~\cite{wei2018revisiting,lee2019ficklenet,mittal2019semi}.
These approaches reduce the dependence on dense annotations but still require large class labeled data for training, which limits their widespread use in real applications.
Contrary to these approaches, the number of weak labeled data required in our method is small (less than 15 per class).

\subsection{Few-shot Learning}
Few-shot learning aims to learn general knowledge that can be applied to learn a novel class with a few examples. Most of the proposed methods are deep meta-learning models, which try to optimize the base learner using learning experiences from multiple similar tasks. One category of existing methods for few-shot learning is gradient-based methods, which aim to adapt the model to a novel class within a few fine-tuning updates~\cite{finn2017model,finn2018probabilistic,jiang2018learning}.
Another category of few-shot learning approaches is metric learning, which learns a metric space across different tasks~\cite{koch2015siamese,vinyals2016matching,sung2018learning}. Prototypical Network~\cite{snell2017prototypical} takes an average over all sample embedding to present each class and performs nearest-neighbor matching to classify data. 


% Our work is mostly related to a semi-supervised prototypical network~\cite{ren2018meta}. It proposes a semi-supervised few-shot learning paradigm by adding an unlabeled set to each episode. This way, the model can augment the support set with unlabeled examples when producing prototypes and meta-learn a better embedding space. Our model follows the semi-supervised few-shot learning paradigm based on Prototypical Network and can be seen as an extension of semi-supervised few-shot learning in a dense form to solve the segmentation task.

\subsection{Few-shot Semantic Segmentation}
The few-shot semantic segmentation task is first solved by using the support branch to predict the weights of the last layer in the query branch~\cite{shaban2017one}. One group of existing works~\cite{zhang2019canet,siam2019amp,zhang2019pyramid} adopt similar idea to match the query image to support pixel-level labeled images. However, these methods mainly address one-way few-shot semantic segmentation task and are computationally expensive to adapt to the multi-way setting.

Another group of the existing approaches are proposed based on metric learning methods~\cite{dong2018few,wang2019panet,nguyen2019feature,liu2020part}, which generate prototypes of semantic classes to match pixels on query images.
% PANet~\cite{wang2019panet} takes the averaged feature embedding in a pixel-level as the class prototype and trains the metric space with prototype alignment constrains between support and query prototypes. 
% PPNet~\cite{liu2020part} is most related to our method. It decomposes object representation into a small set of part-aware prototypes and leverages extra image-level annotations to enrich prototypes. 
Recently, ~\cite{liu2020part} proposed PPNet method to leverage extra image-level annotations to enrich prototypes.
Despite the similarity, it differs from our work in the two aspects: 1) All pixels that are predicted to be related share the same weights to generate region-level features of image-level annotations.
Instead, our work considers the uncertainty of the prediction with a soft-masked pooling strategy; 2) It first selects the relevant parts by a pre-defined threshold while our model generates the task-specific filter threshold to handle the noise, which improves the utilization of the data and robustness of the method.
% , which limits the utilization of the image-level annotations and the knowledge extraction capability of the model.
